Unsupervised Topic Discovery in User Comments

On social media platforms like Twitter, users regularly share their opinions and comments with software vendors and service providers. Popular software products might get thousands of user comments per day. Research has shown that such comments contain valuable information for stakeholders, such as feature ideas, problem reports, or support inquiries. However, it is hard to manually manage and grasp a large amount of user comments, which can be redundant and of a different quality. Consequently, researchers suggested automated approaches to extract valuable comments, e.g., through problem report classifiers. However, these approaches do not aggregate semantically similar comments into specific aspects to provide insights like how often users reported a certain problem. We introduce an approach for automatically discovering topics composed of semantically similar user comments based on deep bidirectional natural language processing algorithms. Stakeholders can use our approach without the need to configure critical parameters like the number of clusters. We present our approach and report on a rigorous multiple-step empirical evaluation to assess how cohesive and meaningful the resulting clusters are. Each evaluation step was peer-coded and resulted in inter-coder agreements of up to 98%, giving us high confidence in the approach. We also report a thematic analysis on the topics discovered from tweets in the telecommunication domain.

==> table/tab_datasource.tex <==
% array([ 84,  64,  63,  61,  36,  68,  48,  34,  36,  61, 108,  83,  30,
%         54,  32,  48,  54,  91, 150,  58,  36,  54,  30,  46,  41,  34,
%         48, 117,  39,  30,  32,  54,  47,  38,  81, 103,  89,  47,  71,
%         42,  51,  38,  89,  41,  82, 105,  56,  75,  75,  56,  31,  45,
%         38,  55,  64,  50,  56,  40, 222,  75,  42,  33,  32,  43,  74,
%         37,  88,  37,  66,  51,  63,  46,  56, 113,  36,  49,  51,  84,
%        121,  58,  56, 132,  41,  45,  92,  41,  30,  62,  55,  60,  32,
%         46,  34,  30,  44,  51,  72,  35,  53,  42, 116,  32,  31,  50,
%         30,  61,  62,  89,  35,  32,  81, 116,  50, 132,  38,  36,  79,
%         77, 115,  52,  95,  54,  48,  36, 122, 125,  93,  53,  77,  69,
%         83,  97,  35, 190, 161, 145,  44,  51,  41, 121, 140,  34, 276,
%        109,  48, 109,  32, 122, 149, 137,  35,  44,  69,  44,  65, 240,
%        244,  79,  75,  56, 204, 201,  51,  36,  57,  42,  62, 145, 127,
%         94,  47,  30,  81,  51,  53,  85,  82,  69,  93, 101, 141,  31,
%         89,  45,  50, 152,  80,  83,  46,  60,  54,  78,  47,  32,  61,
%         34,  35,  36,  40,  30,  48,  76,  42,  47,  42,  83,  36,  33,
%         63,  38,  35,  74,  31, 128,  49,  45,  59,  35,  97,  72, 115,
%         30,  40,  41,  47,  35,  35,  64,  40, 467,  35, 127,  51, 259,
%         41,  94,  48,  45,  30,  57, 187,  32,  35, 123, 207,  93,  84,
%         41, 108,  45,  42,  36, 110,  61,  33,  76,  38,  31,  32,  30,
%         44,  47, 160,  59,  45,  88,  37,  34,  48,  64,  87,  96,  41,
%         41, 168,  38,  95,  41,  38,  60,  98,  37,  50,  46, 212,  61,
%         41,  47,  81,  44,  38, 559,  45,  60,  71,  45,  42, 589,  42,
%         34,  32, 107,  77,  81, 145,  54, 128,  82,  40,  80,  43,  32,
%         61,  43, 144,  32,  31,  91, 126, 150,  35, 223,  51,  76,  46,
%        140,  32,  67, 111,  56,  44,  39, 150,  90,  62,  50, 158, 313,
%         38,  31,  32,  30,  45,  30,  36, 397, 158,  39,  37,  75,  37,
%         43, 198,  41,  47,  82,  57,  46,  37,  61,  85,  37, 102,  30,
%        486,  65,  60, 111,  69,  52,  43,  65,  68,  70,  92,  43,  86,
%         50,  98,  31,  66, 266, 285,  68,  69,  31, 195,  69,  57, 108,
%        128,  48,  97, 105,  34,  63,  42, 208,  44,  41,  92,  36,  89,
%         40,  30,  52,  71,  70,  52,  37,  87, 140,  68,  53, 152,  87,
%         36,  39,  52,  63,  52,  44,  38, 101, 100,  52])


\begin{table}[tb]
\centering
    \footnotesize
    \caption{Descriptive statistics of the collected data.}
\begin{tabular}{lr}
\toprule
                                  & Value \\ \midrule
\rc Data source         & Twitter \\
    Domain              & Telecommunication \\
\rc n\_datapoints       & 138,639 \\
    n\_clusters         & 425 \\
\rc cluster size        & \(76 \pm 65\) (\(\mu \pm \sigma\)) \\
    avg. cluster length & x \\ \bottomrule
\end{tabular}
  \label{tab:descriptive_statistics}
\end{table}

==> table/tab_results_expert_labels_scoring_examples.tex <==
\begin{table}[tb]
\centering
    \footnotesize
    \caption{Examples for agreements and disagreements in expert label attribute descriptions}
\begin{tabular}{@{}lllr@{}}
\toprule
\textbf{Attribute} & \textbf{Annotaton A}              & \textbf{Annotation B}         & \textbf{Agreement Score} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
Concern            & Network status inquiry            & Details about network problem & 1                        \\
Trigger            & reponse from the Twitter(support) & Response from support         & 1                        \\
\rowcolor[HTML]{EFEFEF} 
Entity             & \#HuaweiP30                       & Huawei P30                    & 1                        \\
Concern            & travel (being outside)            & Resolutions                   & 0                        \\
\rowcolor[HTML]{EFEFEF} 
Emotion            & positive                          & neutral                       & 0                        \\
Concern            & -                                 & Buy, Trade-In                 & 0                        \\ \bottomrule
\end{tabular}
\label{tab:results:expert_labels:scoring_examples}
\end{table}

